Measurement of the t dependence in exclusive photoproduction of Upsilon(1S) mesons at HERA

The exclusive photoproduction reaction gamma p -> Upsilon(1S) p has been studied with the ZEUS detector in ep collisions at HERA using an integrated luminosity of 468 pb^-1. The measurement covers the kinematic range 60<W<220 GeV and Q^2<1 GeV^2, where W is the photon-proton centre-of-mass energy and Q^2 is the photon virtuality. The exponential slope, b, of the t dependence of the cross section, where t is the squared four-momentum transfer at the proton vertex, has been measured, yielding b = 4.3 +2.0 -1.3 (stat.) +0.5 -0.6 (syst.) GeV^-2. This constitutes the first measurement of the t dependence of the gamma p -> Upsilon(1S) p cross section.

==> DESY-11-186-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{./BiBTeX/user/syn.bib,%
             ./BiBTeX/bib/l4z_articles.bib,%
             ./BiBTeX/bib/l4z_books.bib,%
             ./BiBTeX/bib/l4z_conferences.bib,%
             ./BiBTeX/bib/l4z_h1.bib,%
             ./BiBTeX/bib/l4z_misc.bib,%
             ./BiBTeX/bib/l4z_old.bib,%
             ./BiBTeX/bib/l4z_preprints.bib,%
             ./BiBTeX/bib/l4z_replaced.bib,%
             ./BiBTeX/bib/l4z_temporary.bib,%
             ./BiBTeX/bib/l4z_zeus.bib}}
}
\vfill\eject

